LAR-IQA: A Lightweight, Accurate, and Robust No-Reference Image Quality Assessment Model

Recent advancements in the field of No-Reference Image Quality Assessment (NR-IQA) using deep learning techniques demonstrate high performance across multiple open-source datasets. However, such models are typically very large and complex making them not so suitable for real-world deployment, especially on resource- and battery-constrained mobile devices. To address this limitation, we propose a compact, lightweight NR-IQA model that achieves state-of-the-art (SOTA) performance on ECCV AIM UHD-IQA challenge validation and test datasets while being also nearly 5.7 times faster than the fastest SOTA model. Our model features a dual-branch architecture, with each branch separately trained on synthetically and authentically distorted images which enhances the model's generalizability across different distortion types. To improve robustness under diverse real-world visual conditions, we additionally incorporate multiple color spaces during the training process. We also demonstrate the higher accuracy of recently proposed Kolmogorov-Arnold Networks (KANs) for final quality regression as compared to the conventional Multi-Layer Perceptrons (MLPs). Our evaluation considering various open-source datasets highlights the practical, high-accuracy, and robust performance of our proposed lightweight model. Code: https://github.com/nasimjamshidi/LAR-IQA.

==> backup.tex <==
A typical multimedia delivery chain consists of multiple stages: content acquisition and encoding, content delivery (via CDNs and ISPs) and decoding and playback at the end user device such as smartphone or TV. However, at each stage, different distortions such as encoding artefacts due to lossy compression, or stalling events due to non-arrival of packets in time etc. can be introduced, which in the end influences the experience of the end user. Assessing the end user experience is imperative for all parties involved to make sure that the user satisfaction is maintained to prevent user churn and/or to attract newer consumers. 

Previously, such experience was assessed based on technical factors such as delay, packet loss, and throughput termed as Key Performance Indicators (KPIs) in the telecommunication industry. These KPIs are monitored continuously or at regular interval to ensure that a certain level of quality as agreed upon in a Service Level Agreement (SLA) is being provided. However, QoS exclusively due to its reliance on pure technical characteristics of telecommunication services for the user’s satisfaction fails to measure the quality from the user perspective. To address this gap, a more human-centric approach to measure quality, termed as QoE in recent years have been introduced which considers a wider range of factors such as content, context and user along with the traditionally used system factors by QoS based measurements.

Quality of Experience is  defined as ``The degree of delight or annoyance of the user of an application or service. QoE is highly subjective as it depends on the user factors (expectations, context, etc.), content, context along with other system and technical factors (network bandwidth, video quality, etc.). This makes estimation of video quality as well as QoE a challenging task as the relevant information and data related to terminal capabilities (e.g., screen size, display performance), application/service specific information and its quantification, QoE-related information inside the network - all have to be monitored, collected and measured \cite{barman_survey,Alex_Survey}. 

\subsection{Motivation}

The new era of QoE led to many efforts towards measuring and modeling QoE that are much closer to human judgment allowing for QoE based monitoring and optimization solutions. Over the years, many different works has been proposed towards QoE modelling \cite{barman_survey}, QoE management of multimedia streaming services in future networks \cite{Alex_Survey} and measuring, modeling and integrating time-varying video quality in end-to-end multimedia service delivery \cite{chaminda_timeVarying}. However, considering the complexity of the multimedia ecosystem as well considering the rapid changes to the underlying technologies from newer codecs (VVC, AV1, LCEVC) \cite{barman2022lcevc} to video formats (HDR, 360, AR/VR), transmission technologies (5G, SDN, NFV), delivery format (multi-tier CDNs, CMAF, etc.) many challenges still remain to develop a holistic QoE model for multimedia applications and services.

